Unusual Hall Effect in Superconducting MgB$_2$ Films: Analogy to High-T$_c$ Cuprates

We have investigated the temperature and magnetic field dependence of the Hall coefficient of two well-characterized superconducting MgB$_2$ films (T$_{c0}$=38.0 K) in both the normal and superconducting states. Our results show that the normal-state Hall coefficient R$_H$ is positive and increases with decreasing temperature, independent of the applied magnetic field. Below T$_c$(H), R$_H$ decreases rapidly with temperature and changes sign before it reaches zero. The position and magnitude at which R$_H$ shows a minimum depends on the applied field. Quantitative analysis of our data indicates that the Hall response of MgB$_2$ behaves very similarly to that of high-T$_c$ cuprates: R$_H$ $\propto$ T and cot$\theta_H$ $\propto$ T$^2$ in the normal state, and a sign reversal of R$_H$ in the mixed state. This suggests that the B-B layers in MgB$_2$, like the Cu-O planes in high-T$_c$ cuprates, play an important role in the electrical transport properties.

==> mgb2bib.tex <==
@ARTICLE{naga,
   author = "J. Nagamatsu and N. Nakagawa and T. Muranaka and y. Zenitani and J. Akimitsu",
   year = "2001",
   journal = "Nature",
   volume = "410",
   pages = "63"

 @ARTICLE{cooper,
    author = "{A.S. Cooper {\it et al.}}",
    year = "1970",
    journal = "Proc. National Acad. Sci. USA",
   volume = "67",
   pages = "313"
}

 @ARTICLE{leya,
   author = "L. Leyarovska and E. Leyvarovski",
   year = "1979",
   journal = "J. Less Common Metals",
   volume = "67",
   pages = "249"
}

@ARTICLE{budko,
   author = "{S.L. Bud'ko {\it et al.}}",
   year = "2001",
   journal = "Phys. Rev. Lett.",
   volume = "86",
   pages = "1877"
   journal = "cond-mat/0102413"
}

@ARTICLE{kara,
    author = "{G. Karapetrov {\it et al.}}",
    year = "2001",
    journal = "cond-mat/0102312"
}

@ARTICLE{sharoni,
   author = "A. Sharoni and I. Felner and O. Millo",
   year = "2001",
   journal = "cond-mat/0102325"
}

@ARTICLE{kote,
   author = "{H. Kotegawa {\it et al.}}",
   year = "2001",
   journal = "cond-mat/0102334"
}

@ARTICLE{tou,
   author = "{H. Tou {\it et al.}}",
   year = "2001",
   journal = "cond-mat/0103484"
}

@ARTICLE{walti,
    author = "Ch. Walti and E. Felder and C. Degen and G. Wigger and R. Monnier and B. Delley and H.R. Ott",
    year = "2001",
    journal = "cond-mat/0102522"
}

@ARTICLE{kremer,
    author = "R.K. Kremer, B.J. Gibson and K. Ahn",
    year = "2001",
    journal = "cond-mat/0102432"
}

@ARTICLE{li,
    author = "{S.L. Li and H.H. Wen and Z.W. Zhao {\it et al.}}",
    year = "2001",
    journal = "cond-mat/0103032"
}

@ARTICLE{pana,
    author = "C. Panagopoulos and B.D. Rainford and T. Xiang and C.A. Scott and M. Kambara and I.H. Inoue",
    year = "2001",
    journal = "cond-mat/0103060"
}

@ARTICLE{zhukov,
    author = "{A.A. Zhukov, K. Yates, G.K. Perkins {\it et al.}}",
    year = "2001",
    journal = "cond-mat/0103587"
}

@ARTICLE{hirsch,
    author = "J.E. Hirsch",
    year = "2001",
    journal = "cond-mat/0102115"
}

@ARTICLE{kang,
    author = "{W.N. Kang, C.U. Jung, K.H.P. Kim {\it et al.}}",
    year = "2001",
    journal = "cond-mat/0102479"
}

@BOOK{anderson,
    author = "P.W. Anderson",
    title = "Theory of Superconductivity in High-T$_c$ Cuprates",
    publisher = "Princeton University Press",
    year = "1997",
    address = "Princeton"
}

 @ARTICLE{para,
    author = "{M. Paranthaman {\it et al.}}",
    year = "2001",
    journal = "Appl. Phys.
 Lett. (in press)"
}

@BOOK{hurt,
    author = "C. Hurd",
    title = "The Hall effect and its applications",
    publisher = "Plenum",
    year = "1980",
    editor = "C.L. Chien and C.R. Westagate",
    address = "New York"
}

@ARTICLE{kortus,
    author = "{J. Kortus {\it et al.}}",
    year = "2001",
    journal = "cond-mat/0101446"
}

@ARTICLE{shul,
    author = "{S.V. Shulga {\it et al.}}",
    year = "2001",
    journal = "cond-mat/0103154"
}

@ARTICLE{kong,
    author = "Y. Kong and O.V. Dolgov and O. Jepsen and O.K. Anderson",
    year = "2001",
    journal = "cond-mat/0102499"
}

@ARTICLE{takano,
    author = "{Y. Takano {\it et al.}}",
    year = "2001",
    journal = "(unpublished)"
}

@ARTICLE{nv,
   author = "P. Nozieres and W.F. Vinen",
   year = "1966",
   journal = "Philos. Mag.",
   volume = "14",
   pages = "667"
}

@ARTICLE{wang,
   author = "{Z.D. Wang {\it et al.}}",
   year = "1994",
   journal = "Phys. Rev. Lett.",
   volume = "72",
   pages = "3875"
}

@ARTICLE{ferr,
   author = "R. Ferrell",
   year = "1992",
   journal = "Phys. Rev. Lett.",
   volume = "68",
   pages = "2524"
}

@ARTICLE{luo,
   author = "{J. Luo {\it et
al.}}",
   year = "1992",
   journal = "Phys. Rev. Lett.",
   volume = "68",
   pages = "690"
}

@ARTICLE{harris,
   author = "{J.M. Harris {\it et
al.}}",
   year = "1994",
   journal = "Phys. Rev. Lett.",
   volume = "73",
   pages = "610"
}

@ARTICLE{feig,
   author = "{M.V. Feigel'man {\it et
al.}}",
   year = "1995",
   journal = "JETP Lett.",
   volume = "62",
   pages = "834"
}

@ARTICLE{dorsey,
   author = "A. Dorsey",
   year = "1994",
   journal = "Phys. Rev. B",
   volume = "46",
   pages = "8376"
}

@ARTICLE{gl,
   author = "V.B. Geshkenbein and A.I. Larkin",
   year = "1994",
   journal = "Phys. Rev. Lett.",
   volume = "73",
   pages = "609"
}

@ARTICLE{kopnin,
   author = "{N.B. Kopnin {\it et al.}}",
   year = "1993",
   journal = "J. of Low Temp. Phys.",
   volume = "90",
   pages = "1"
}

